Dark-ISP: Enhancing RAW Image Processing for Low-Light Object Detection

Low-light Object detection is crucial for many real-world applications but remains challenging due to degraded image quality. While recent studies have shown that RAW images offer superior potential over RGB images, existing approaches either use RAW-RGB images with information loss or employ complex frameworks. To address these, we propose a lightweight and self-adaptive Image Signal Processing (ISP) plugin, Dark-ISP, which directly processes Bayer RAW images in dark environments, enabling seamless end-to-end training for object detection. Our key innovations are: (1) We deconstruct conventional ISP pipelines into sequential linear (sensor calibration) and nonlinear (tone mapping) sub-modules, recasting them as differentiable components optimized through task-driven losses. Each module is equipped with content-aware adaptability and physics-informed priors, enabling automatic RAW-to-RGB conversion aligned with detection objectives. (2) By exploiting the ISP pipeline's intrinsic cascade structure, we devise a Self-Boost mechanism that facilitates cooperation between sub-modules. Through extensive experiments on three RAW image datasets, we demonstrate that our method outperforms state-of-the-art RGB- and RAW-based detection approaches, achieving superior results with minimal parameters in challenging low-light environments.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


% How to refer a paper \cite{gao2025deep}.
% 1. 在google scholar上搜索，选择引用，选择bibtex格式，复制到main.bib里
% 2. bibtex格式的第一个就是这篇文章的label，也可以换，正文就用\cite{label}就行

% 第一段：点出Object detection + low-light重要但很难
Object detection plays a vital role in computer vision applications like autonomous driving and surveillance systems.\ref{girshick2015fast}\ref{girshick2015fast}\ref{girshick2015fast} While deep learning advances have significantly boosted detection accuracy in normal lighting, low-light scenarios remain challenging due to two fundamental limitations: insufficient photon capture by sensors and amplified noise during image signal processing (ISP). These issues corrupt critical visual features, severely degrading existing detection methods in practical low-light environments [...].

% 第二段：现在的方法怎么做的，RGB方法不行，是使用Raw images的隐藏动机，这一段少写一点
%The majority of researches focus on utilizing low-light RGB images combined with meticulously designed enhancement modules as preprocessing steps or introducing feature-level operation at intermediate stages of the network.[  Some dark RGB methods  ]However, due to the limited valid information contained in low-bit-depth RGB images under dark conditions, as well as the noise introduced during  process of electronic imaging [physical noise] and image processing pipeline (ISP)[......], the potential of the aforementioned approaches is significantly constrained, resulting in a heavy reliance on designing complex training pipelines and network architectures to optimize performance. Their effectiveness remains inherently limited and faces notable bottlenecks.
To address low-light detection, most approaches process dark RGB images through enhancement modules or network architecture modifications [Some dark RGB methods]. However, such RGB-based methods face inherent bottlenecks: (1) the limited bit-depth (typically 8-bit) of post-ISP RGB data discards photon-level details crucial for low-light analysis; (2) sensor defects and ISP nonlinear operations introduce compounded noise that preprocessing struggles to suppress [...]. Consequently, these methods resort to intricate training pipelines or bulky networks with diminishing returns, evidenced by persistent failure cases in real deployments [...]. 

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/Comparison.pdf} 
\caption{The thumbnail of different low-light object detection pipline. (a) Methods utilizing RGB-RAW data. (b) ISP parameter search methods. (c) Methods introducing auxiliary information for training. (d) Dark RGB image enhancement pipline. (e) The proposed pipline.}
\label{fig:comparsion}
\end{figure}

% 第三段：现在的方法怎么做的，Raw images方法初显实力，但也还不够好，有值得改进的地方
% 这一段内部结构没有formulate的很好，可以再改改，或者我等下改改，而且太长了
% As shown in \cref{fig:comparsion}, a line of works [LIS (CVPR 2018), DynamicISP (ICCV 2023), and Craft (2023)] directly employs RAW images captured in low-light conditions as inputs for detection task, highlighting the advantages of RAW images in dark environment. Nevertheless, these approaches compress the original four-channel Bayer format into three-channel RGB format before feeding them into the network. This coupled with a reduction in bit depth, leads to substantial information loss, ultimately failing to fully exploit the rich informational potential of RAW images. 
% Additionally, there also have a number of studies [NOD (CVPR 2022), AdaptiveISP (NeurIPS 2024), ALHP (ECCV 2022), RAW-Adapter (ECCV 2024)]directly use Bayer-format RAW images as inputs by designing learnable ISP modules to serve as a "bridge" between the RAW and RGB domains. While these approaches successfully exploit the high bit-depth characteristics of RAW images and fully leverage pre-trained backbone parameters for downstream tasks, they often require complex parameter search algorithms or multi-stage training processes, which would be computationally intensive and challenging to implement. Furthermore, other methods [TeacherISP (AAAI 2024) and Multitask AET (ICCV 2021)] incorporate some auxiliary information, such as RGB images under normal lighting conditions or camera parameters, to assist in network training. These approaches often involve relatively intricate architectural designs. Moreover, due to the difficulty in obtaining genuine RAW datasets, some of them resort to using synthetic RAW images as substitutes, which cannot perfectly replicate the noise distribution of real RAW images, thereby constraining their practical applicability and effectiveness. 

Recent approaches exploring RAW-based detection methods have gained attention in the community, as RAW images offer superior performance potential compared to traditional RGB images, due to their higher bit-depth and richer informational content. These methods can be categorized into three paradigms:
(a) Direct RAW Conversion:  Techniques like [LIS (Craft (2023), CVPR 2018), RAW-Adapter] convert the four-channel Bayer format into a three-channel RGB format before feeding them into neural networks. This conversion, combined with bit-depth reduction, causes significant information loss, limiting the ability to fully exploit the rich informational potential of RAW images.
(b) Learnable ISP Bridging: Methods such as [NOD (CVPR 2022), AdaptiveISP (NeurIPS 2024), ALHP (ECCV 2022), and DynamicISP (ICCV 2023) (ECCV 2024)] directly use Bayer-format RAW images by incorporating learnable ISP modules to bridge the RAW and RGB domains. These approaches effectively leverage the high bit-depth of RAW images and pre-trained backbone models, but they require computationally intensive processes, including complex parameter search [...] and multi-stage training [...], which complicate implementation.
(c) Auxiliary Information Augmentation: Methods like TeacherISP [...] and Multitask AET (ICCV 2021)] incorporate normal-light RGB references or camera metadata during training. However, the reliance on synthetic RAW data (which may not align with real sensor noise distributions) or unavailable metadata limits their practical scalability.

% 而且你缺少你自己方法设计的Motivation，就是针对现在的Limitation，你就直接下一段就是你的方法了，challenge=>limitation=>design in your method=>experiments validation应该严密耦合

% 第四段：针对这些缺点，gap，我们提出来怎么样的解决措施
% 这段有点乱
% Considering the strengths and limitations of the aforementioned methods, we propose a straightforward and readily deployable ISP plugin in order to align Bayer RAW format inputs with downstream RGB pre-trained backbone weights facilitating the end-to-end training, as illustrated in \cref{fig:comparsion}(e). To fully integrate the ISP process with the flexible and highly adaptive nature of deep learning, enabling the model to determine how to process RAW images only based on the guidance of downstream task loss, we categorize the camera's original ISP pipeline into linear and nonlinear components according to their functionalities. In the linear component, we integrate the camera's white balance (WB) and color correction matrix (CCM) as prior conditions into the training process. These priors interact with the image data to produce task-specific linear transformations for the ISP through the Attention mechanism[Transformer]. In the nonlinear component, we introduce a set of mapping curves tailored for low-light environments. These curves are dynamically weighted and combined by the network learning to approximate the optimal nonlinear function. Moreover, we propose a self-supervised loss that leverages the output data from the nonlinear component to generate pseudo linear transformation, thereby optimizing the learning of the linear component. The entire training process requires no additional manual annotations,  solely requiring the object detection labels. 

% The main contributions of this work can be summarized as follows:
% \begin{enumerate}[leftmargin=0.6cm]
%     \item We propose a pipeline capable of end-to-end training of visual perception networks using Bayer-format images as input.
%     \item To enable adaptive adjustment of camera parameters based on the loss of downstream perception tasks, we design a learnable ISP linear module.
%     \item Based on the understanding of tone mapping curves in low-light environments, we design pixel-wise and higher-order mapping curves to replace the nonlinear operations in the ISP process.
%     \item Leveraging the sequential structure of the proposed ISP module, we introduce a self-supervised loss as a regularization term to enhance the model's learning capability.
%     \item Without significantly increasing computational overhead, we validate the effectiveness of our approach on several low-light RAW image object detection datasets. Extensive experiments demonstrate that, compared to previous RGB-RAW and RGB end-to-end methods, our approach achieves superior performance while utilizing the fewest parameters.
% \end{enumerate}


